DRAT Proofs of Unsatisfiability for SAT Modulo Monotonic Theories

Generating proofs of unsatisfiability is a valuable capability of most SAT solvers, and is an active area of research for SMT solvers. This paper introduces the first method to efficiently generate proofs of unsatisfiability specifically for an important subset of SMT: SAT Modulo Monotonic Theories (SMMT), which includes many useful finite-domain theories (e.g., bit vectors and many graph-theoretic properties) and is used in production at Amazon Web Services. Our method uses propositional definitions of the theory predicates, from which it generates compact Horn approximations of the definitions, which lead to efficient DRAT proofs, leveraging the large investment the SAT community has made in DRAT. In experiments on practical SMMT problems, our proof generation overhead is minimal (7.41% geometric mean slowdown, 28.8% worst-case), and we can generate and check proofs for many problems that were previously intractable.

==> backup_expeval/evaluation.old.tex <==
\section{Proof Support Workflow and Implementation}
\label{sec:workflow}
\sam{We will likely have to shrink or remove this section to make room for the Tiros results}
% In this section, we illustrate our framework for supporting DRAT proofs in MonoSAT. We first present the overall workflow for generating and verifying the DRAT-style UNSAT proof for MonoSAT, and then discuss the implementation details for the workflow.

We instantiated our proof support framework for MonoSAT. 
%
The work flow is shown in Fig.~\ref{fig:workflow}. 
%
Given an input gnf instance (input formula for MonoSAT), we extended \textit{MonoSAT} to emit a DRAT-style proof certificate that contains theory lemmas (as explained in Sect.~\ref{sec:overview}). 
%
The proof certificate is then processed by \textit{drat-trim-theory}, a modified version of drat-trim that runs \textsc{BackwardCheck}, to extract the core lemmas. For every theory predicate involved in the core lemmas, the \textit{proof generator} encode its propositional definition based on the predicate's monotone circuit (as shown in Sect.~\ref{sec:verifyTheory}). These definitoins are used to expand the original theory predicates in the gnf formula to formulate an eq-satisfiable CNF formula. Finally, we use the unmodified drat-trim~\cite{wetzler2014drat} to check the core lemmas (as a DRAT proof) on the CNF formula and return the result of the verification.
\pt{Did not introduce "gnf" before. It seems like an irrelevant detail that can be easily dropped without confusion.}

% The workflow for supporting the DRAT proof for MonoSAT is depicted in Fig.~\ref{fig:workflow}. Given an input gnf instance (input formula for MonoSAT), we extended \textit{MonoSAT} to emit a DRAT-style proof certificate that contains theory lemmas (as explained in Sect.~\ref{sec:overview}). The proof certificate is then processed by \textit{drat-trim-theory}, a modified version of drat-trim that runs Alg.~\ref{alg:check}, to extract the core lemmas, a subset of lemmas from the certificate which are sufficient as a DRAT proof if theory lemmas are assumed valid. For every theory predicate involved in the core lemmas, the \textit{proof generator} encode its propositional definition based on the predicate's monotone circuit (as shown in Sect.~\ref{sec:verifyTheory}). The propositional definitions for the predicates are then used to expand the original theory predicates in the gnf formula to formulate an eq-satisfiable CNF formula. Finally, we use the unmodified drat-trim~\cite{wetzler2014drat} to check the core lemmas (as a DRAT proof) on the CNF formula and return the result of the verification.

% The whole workflow can be broken down into three stages: (1) Solving with certificate (MonoSAT), (2) generating DRAT proofs (drat-trim-theory and proof generator), and (3) DRAT verification (drat-trim). We will evaluate their respective performance against the raw MonoSAT solving cost in Sect.~\ref{sec:evaluation}. 

\pt{I would rewrite the following paragraph dropping any reference to lines of code, which is a rather imprecise and uninformative measurement. It's more distracting than anything else.}
% To allow MonoSAT to emit proof certificate, we modified the solver with about 100 lines of C++ code. The solver supports emitting certificates in both plain text and binary mode. We implemented Alg.~\ref{alg:check} in drat-trim-theory by extending the drat-trim with less than 50 lines of C code. The proof generator was implemented with about 2000 lines of Python code that includes the monotone circuits for graph reachability and bit-vector comparison. 
%All tools are publicly available~\footnote{Place Holder}.


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{unsat_proof_wf.pdf}
    \caption{The workflow for generating and verifying DRAT proof for MonoSAT. Inputs to the workflow (instance gnf file and monotone circuits) are colored in blue. The new (proof generator) and modified components (MonoSAT and drat-trim-theory) are colored in yellow. The whole workflow can be broken down into three stages: (1) Solving with certificate (MonoSAT), (2) generating DRAT proofs (drat-trim-theory and proof generator) and (3) DRAT verification (drat-trim).}
    \label{fig:workflow}
\end{figure}


\section{Experimental Evaluation}
\label{sec:evaluation}


% Can re-use some text from introduction to set up the two experiments.

In this section, we evaluate our framework's (on MonoSAT) performance with two independent sources of benchmarks: an industrially-provided (by Intel), but publicly-available generator of
VLSI routing challenge problems~\cite{DBLP:conf/fmcad/Nadel16},
and a large set of proprietary UNSAT instances generated
from production use of MonoSAT at Amazon Web Services. 

As mentioned in Sect.~\ref{sec:workflow}, the workflow for supporting the DRAT proof has three stages: (1) solving with certificate, (2) DRAT proof generation, and (3) DRAT proof verification. Therefore, for each instance, we compare the raw MonoSAT solving time with (1) the overhead of emitting the proof certificate (in binary mode), (2) the cost of generating the UNSAT proof, and (3) the final cost of DRAT proof checking. 

\input{tiros}

==> expeval_intro.tex <==
\section{Experimental Evaluation}
\label{sec:evaluation}

In this section we evaluate our framework's (on MonoSAT) performance using
two sets of unsatisfiable network reachability benchmarks.

In its most simplistic formulation, network reachability can be described as the
problem of determining when a given pair of network resources, namely a source and
a destination, can establish a network connection.
%
When the space of possible network packets entailed by the network reachability problem
is very large, the ability to represent network packet completely symbolically makes
SAT-based automated reasoning a competitive technique at large scale.
%
Nowadays, large-scale industrial-level organizations such as Amazon AWS offer
a plethora of widely adopted commercial applications using SAT-based network
reachability analysis (e.g. Amazon Inspector, Amazon VPC Reachability Analyzer
and Amazon VPC Network Access Analyzer).

One possible SAT encoding of the network reachability problem, such as the one
used by Tiros~\cite{backes2019reachability,bayless2021debugging}, relies on the
the Theory of Bit-Vectors and the Theory of Graph Reachability. Both theories
are supported by the framework presented in Section \ref{sec:workflow}, which
constructs monotone circuits as described in Section \ref{sec:buildEncoding}.
%
In this encoding, the network packets involved in the connection handshake
are symbolically represented using Bit-Vectors, and the network is modeled
as a graph, where nodes and edges correspond to real-world network components
and direct "wires" between them respectively.
%
In the real-world, network components can intercept, transform and optionally
re-transmit packets traveling through the network (e.g. a firewall or a NAT
gateway). Network components come in various types, each with its own complex
behavior and rich list of user-configurable network controls. Such behavior
is modeled in terms of a logical function that expresses the relationship
between incoming and outgoing packets for each element of the network graph.


In the real-world network, network reachability is infeasible when for all possible 
packet headers that the source could generate, and for all possible paths connecting
the source to the destination, the combined effect of packet transformations and
network controls placed along the path cause the packet to be eventually dropped
from the network before it reaches the intended destination (e.g. a firewall rule
dropping traffic).
In this case, the framework presented in Section \ref{sec:workflow} of this paper
can be used to verify the proof of unsatisfiability generated by the SMT solver,
drastically boosting the confidence in the correctness of the result.

We ran both experimental evaluations on a {\sf m5.24xlarge} EC2 Instance running
{\sf Amazon Linux 2} with $16$GB or RAM, using a timeout of $1$ hour.
We evaluate the following configurations: {\sc MonoSAT} and {\sc Bit-Blasting}.
The former implements the framework described in Section \ref{sec:workflow}.
The latter eagerly bit-blasts each instance \nf{NF: we can cite Sam's thesis Section 5.2.1 for the method of bit-blasting} into SAT and solves it
with the state-of-the-art SAT solver {\sc Kissat} \cite{fleury2020cadical}.
%
In both cases, the proof is verified with {\sc DRAT-trim} \cite{DBLP:conf/sat/WetzlerHH14}.

The goal of these experiments is to demonstrate that the framework described in
Section \ref{sec:workflow} can scale better than a naive {\sc Bit-Blasting}
approach. 

\pt{Dangling bibliographic references}


\input{tables/expeval_joint_stats_figs}

\input{expeval_public}

\input{expeval_tiros}





==> expeval_public.tex <==
\subsection{Public Network Reachability Benchmarks}
\label{sec:evaluation_public}

In this experiment we evaluate the framework in Section \ref{sec:workflow} on a set
of artificially generated benchmarks that reproduce, without disclosing any critical
industrial information, the real-world problems solved by Tiros~\cite{backes2019reachability,bayless2021debugging}
on behalf of Amazon VPC Reachability Analyzer.

Each benchmark contains an instance of the network reachability problem over a
network topology that can contain only two types of intermediate components:
simple and transforming ones.
%
Simple network components relay an incoming packet as long as its destination address
belongs to a certain domain, expressed in terms of a network CIDR (e.g. 10.0.0.0/24).
%
Transforming network components intercept an incoming packet and rewrite the
source address and ports to match their own before re-transmitting it.
%
At an intuitive level, simple network components are akin to Subnets, VPCs and
Peering Connections in the real-world setting, whereas transforming network
components can be thought of as an overly simplified version of Load Balancers,
NAT Gateways, Network Firewalls, etc.
%
Because for the purposes of this experimental evaluation we are only interested in
unsatisfiable network reachability instances, we restrict the set of network packets
accepted by the final destination so that no matter which combination of transforming
network components it is visited, the packet is not accepted.
%
This emulates real-world network connectivity issues caused by overly restrictive
network controls (e.g. a firewall) and improperly configured intermediate components
(e.g. a load balancer with an incorrect target).

We generated $24$ instances in total, varying the size and structure of the randomly
generated network, and we made them publicly available here \cite{public_network_bench}.
%
We empirically verified that generating the proof of unsatisfiability
for the benchmarks so obtained, requires roughly the same amount of time as the average
real-world problems solved by Tiros for the industrial application. Using these
proofs of unsatisfiability, we evaluated the framework presented in this paper.

The results are shown in Figure \ref{fig:expeval_stats} (table and top row).
%
Looking at the data in the table, we observe that both {\sc MonoSAT} and {\sc Bit-Blasting}
incur in timeouts ($5$ and $16$ resp.) and out-of-memory errors ($5$ and $3$ resp.). Overall,
using {\sc MonoSAT} we were able to solve and prove $9$ more instances than with the other
approach.
Looking at the scatter plot comparison, we can see that {\sc MonoSAT} solves the instances
in this benchmark-set up to an order of magnitude faster than {\sc Bit-Blasting} and that
{\sc DRAT-trim} is able to verify the proof of unsatisfiability up to $50\%$ faster for
the {\sc MonoSAT} configuration.
%
Overall, verifying the proof of unsatisfiability takes at least an order of magnitude longer
than solving the original instances, with either configuration.



==> expeval_tiros.tex <==
\subsection{Tiros Network Reachability Benchmarks}
\label{sec:evaluation_tiros}

In this experiment we evaluate the framework in Section \ref{sec:workflow} on a set
of real-world problems%
\footnote{The benchmark-set cannot be disclosed because it contains critical details for the industry.}
solved by Tiros~\cite{backes2019reachability,bayless2021debugging}
on behalf of Amazon VPC Reachability Analyzer.


The results are shown in Figure \ref{fig:expeval_stats} (table and bottom row).
%
Looking at the data in the table, we observe that both {\sc MonoSAT} and {\sc Bit-Blasting}
incur in timeouts ($4$ and $19$ resp.) and out-of-memory errors ($98$ and $102$ resp.). Overall,
using {\sc MonoSAT} we were able to solve and prove $19$ more instances than with the other
approach.
%
% On average, {\sc MonoSAT} was also over an order of magnitude faster at solving
% instances and two order of magnitude faster when verifying proofs.
%
Looking at the scatter plot comparison, we can identify a subset of problems that
are able to terminate with the {\sc MonoSAT} but not with the {\sc Bit-Blasting}
configurations and another subset of problems in which the converse case applies.
%
When the evaluation terminates successfully with both configurations, {\sc MonoSAT}
outperforms {\sc Bit-Blasting} by up to two orders of magnitude when solving the
instance and one order of magnitude when {\sc DRAT-trim} is used to verify the proof
of unsatisfiability.


==> tables/expeval_joint_stats.tex <==
\begin{table}[tb]
\scriptsize
\centering
\begin{tabularx}{\textwidth}{|X|r|r|r|r|r|r|r|r|r|}
\cline{2-9}
\multicolumn{1}{c}{}               &
\multicolumn{4}{|c|}{\bf Count}    &
\multicolumn{2}{c|}{\bf Time (s.)} &
\multicolumn{2}{c|}{\bf Count}     &
\multicolumn{1}{c}{\bf }        \\
\cline{1-9}
\multicolumn{1}{|c|}{\bf config.} &
\multicolumn{1}{c|}{\bf total}          &
\multicolumn{1}{c|}{\bf timeout}        &
\multicolumn{1}{c|}{\bf OOM}         &
\multicolumn{1}{c|}{\bf success}        &
\multicolumn{1}{c|}{\bf Solve}   &
\multicolumn{1}{c|}{\bf Proof}   &
\multicolumn{1}{c|}{\bf T. Lem.}     &
\multicolumn{1}{c|}{\bf Oblig.}   &
\multicolumn{1}{c}{\bf }   \\
\cline{1-9}\noalign{\vspace{0.75ex}}
\hline
% Public Network Reachability Benchmarks
\multicolumn{10}{|l|}{\cellcolor{black!15}\textbf{Public Network Reachability Benchmarks}}\\
\hline
\hline
{\sc Bit-Blasting} & 24 & 16 & 3 & 5 & 805 & 8203 & - & - & {\bf sum} \\
                   &    &    &   &   & 161 & 1641 & - & - & {\bf mean} \\
%|bitblasting|   mean|        161|       1641|
%|bitblasting| median|        151|       1525|
%|bitblasting|    P99|        287|       2590|
%|bitblasting|    sum|        805|       8203|
\hline
{\sc MonoSAT}     & 24 & 5 & 5 & {\bf 14} & 340 & 18789 & - & - & {\bf sum} \\
                  &    &   &   &          & 24 &  1342 & 266 & 118 & {\bf mean} \\
%|MonoSAT    |   mean|         24|       1342|
%|MonoSAT    | median|         22|        988|
%|MonoSAT    |    P99|         40|       2813|
%|MonoSAT    |    sum|        340|      18789|
\hline
\hline
% Tiros Network Reachability Benchmarks

\multicolumn{10}{|l|}{\cellcolor{black!15}\textbf{Tiros Network Reachability Benchmarks}}\\
\hline
{\sc Bit-Blasting} & 255 & 19 & 102 & 134 & 16249 & 59610 & - & - & {\bf sum} \\
                   &     &    &     &     & 121 &   445 & - & - & {\bf mean} \\
%|bitblasting|   mean|        121|        445|
%|bitblasting| median|        117|        323|
%|bitblasting|    P99|        307|       2028|
%|bitblasting|    sum|      16249|      59610|
\hline
{\sc MonoSAT}     & 255 &  4 & 98 & {\bf 153} & 546 & 8833 & - & - & {\bf sum} \\
                  &     &    &    &           & 4 &   58 & 2602 & 11 & {\bf mean} \\
%|MonoSAT    |   mean|          4|         58|
%|MonoSAT    | median|          2|         51|
%|MonoSAT    |    P99|         55|        268|
%|MonoSAT    |    sum|        546|       8833|
\hline
\end{tabularx}
\caption[Experimental Results]{\label{tab:expeval_stats}
Experimental results for both benchmark-sets, showing best performer in {\bf boldface}. Timing results include
successful benchmarks only.
}
\end{table}

==> tables/expeval_joint_stats_figs.tex <==
\begin{figure}[!t]
%\centering
%\begin{table}[tb]
\scriptsize
\centering
\begin{tabularx}{\textwidth}{|X|r|r|r|r|r|r|r|r|r|}
\cline{2-9}
\multicolumn{1}{c}{}               &
\multicolumn{4}{|c|}{\bf Count}    &
\multicolumn{2}{c|}{\bf Time (s.)} &
\multicolumn{2}{c|}{\bf Count}     &
\multicolumn{1}{c}{\bf }        \\
\cline{1-9}
\multicolumn{1}{|c|}{\bf config.} &
\multicolumn{1}{c|}{\bf total}          &
\multicolumn{1}{c|}{\bf timeout}        &
\multicolumn{1}{c|}{\bf OOM}         &
\multicolumn{1}{c|}{\bf success}        &
\multicolumn{1}{c|}{\bf Solve}   &
\multicolumn{1}{c|}{\bf Proof}   &
\multicolumn{1}{c|}{\bf T. Lem.}     &
\multicolumn{1}{c|}{\bf Oblig.}   &
\multicolumn{1}{c}{\bf }   \\
\cline{1-9}\noalign{\vspace{0.75ex}}
\hline
% Public Network Reachability Benchmarks
\multicolumn{10}{|l|}{\cellcolor{black!15}\textbf{Public Network Reachability Benchmarks}}\\
\hline
{\sc Bit-Blasting} & 24 & 16 & 3 & 5 & 805 & 8203 & - & - & {\bf sum} \\ %& 24 & 19 & 0 & 5 & 805 & 8203 & - & - & {\bf sum} \\
                   &    &    &   &   & 161 & 1641 & - & - & {\bf mean} \\
%|bitblasting|   mean|        161|       1641|
%|bitblasting| median|        151|       1525|
%|bitblasting|    P99|        287|       2590|
%|bitblasting|    sum|        805|       8203|
\hline
{\sc MonoSAT}     & 24 & 5 & 5 & {\bf 14} & 340 & 18789 & - & - & {\bf sum} \\ %& 24 & 10 & 0 & {\bf 14} & 340 & 18789 & - & - & {\bf sum} \\
                  &    &   &   &          & 24 &  1342 & 266 & 118 & {\bf mean} \\
%|MonoSAT    |   mean|         24|       1342|
%|MonoSAT    | median|         22|        988|
%|MonoSAT    |    P99|         40|       2813|
%|MonoSAT    |    sum|        340|      18789|
\hline
\hline
% Tiros Network Reachability Benchmarks

\multicolumn{10}{|l|}{\cellcolor{black!15}\textbf{Tiros Network Reachability Benchmarks}}\\
\hline
{\sc Bit-Blasting} & 255 & 19 & 102 & 134 & 16249 & 59610 & - & - & {\bf sum} \\ %& 255 & 89 & 17 & 149 & 17967 & 74466 & - & - & {\bf sum} \\
                   &     &    &     &     & 121 &   445 & - & - & {\bf mean} \\ %&     &    &     &     & 121 &   500 & - & - & {\bf mean} \\
%|bitblasting|   mean|        121|        445|
%|bitblasting| median|        117|        323|
%|bitblasting|    P99|        307|       2028|
%|bitblasting|    sum|      16249|      59610|
\hline
{\sc MonoSAT}     & 255 &  4 & 98 & {\bf 153} & 546 & 8833 & - & - & {\bf sum} \\ %& 255 &  68 & 31 & {\bf 156} & 613 & 11638 & - & - & {\bf sum} \\
                  &     &    &    &           & 4 &   58 & 2602 & 11 & {\bf mean} \\ %&     &    &    &           & 4 &   75 & 2650 & 11 & {\bf mean} \\
%|MonoSAT    |   mean|          4|         58|
%|MonoSAT    | median|          2|         51|
%|MonoSAT    |    P99|         55|        268|
%|MonoSAT    |    sum|        546|       8833|
\hline
\end{tabularx}
%\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vspace{1.0em}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{tabular}{cc}%
\hspace{-1em}
            %\includegraphics[scale=0.55]{plots/key_flow_bench_new_monosat_default_bitblasting_solve_times.png}
		\includegraphics[scale=0.55]{plots/public_solve_new.png}
&
\hspace{-1em}
            %\includegraphics[scale=0.55]{plots/key_flow_bench_new_monosat_default_bitblasting_proof_times.png}\\
		\includegraphics[scale=0.55]{plots/public_proof_new.png}\\

\hspace{-1em}
		\includegraphics[scale=0.55]{plots/tiros_solve_new.png}
            %\includegraphics[scale=0.55]{plots/monosat_default_bitblasting_solve_times.png}
&
\hspace{-1em}
            %\includegraphics[scale=0.55]{plots/monosat_default_bitblasting_proof_times.png}\\
		\includegraphics[scale=0.55]{plots/tiros_proof_new.png}\\
\end{tabular}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\caption[Experimental Results]{\label{fig:expeval_stats}
[Table] Experimental results for both benchmark-sets, showing best performer in {\bf boldface}. Timing results include
successful benchmarks only.
[Top row] Pairwise comparison on the Public Network Reachability Benchmarks in Section \ref{sec:evaluation_public}.
[Bottom row] Pairwise comparison on the Tiros Network Reachability Benchmarks in Section \ref{sec:evaluation_tiros}. 
Green line denotes timeouts, blue line denotes out-of-memory errors.
}
\end{figure}

==> vlsi_results_unused.tex <==
% This section is no longer being included in the paper
% keeping it here for reference

\subsection{Industrial VLSI Routing Problems}

The industrial VLSI Routing under constraints problems (RUC) aim to find a route for every routing group in a hardware board, represented by a $M \times M$ grid-like graph. For simplicity, the problem assumes that every routing group has exactly two end-points, and a route is a path connecting the two end-points using the edges in the graph. Furthermore, the problem requires that every node in the graph belongs to at most one route, since the routes should not interfere with each other (the short rule~\cite{DBLP:conf/dac/TaylorP07}). To cope with other hardware design requirements, additional constraints might be placed on the graph. Inspired by the crafted instances of~\cite{DBLP:conf/fmcad/Nadel16}, we considered binary mutual exclusion constraints between the nodes in the graph such that at most one of the nodes is available for routing. 

Given an instance of the RUC problem
 for finding routes between $N$ groups on a $M \times M$ grid-like graph under $C$ number of binary exclusion constraints, we can encode the problem as a constraint satisfiability problem with graph reachability theory and use MonoSAT to determine its satisfiability. To evaluate our framework for UNSAT proof support, we randomly sample 10 
 UNSAT instances with three different set of parameters configurations: (1) $N=5, M= 10, C \in [40, 50]$,  (2) $N=5, M=20, C \in [600, 800]$ and (3) $N =5, M =30, C \in [3000, 5000]$~\footnote{The the value of $C$ used in ~\cite{DBLP:conf/fmcad/Nadel16} is significantly smaller because they are interested generating SAT instances whereas we are interested in UNSAT instances.}. 

For each sampled UNSAT instance, we launch MonoSAT with proof support, generate the DRAT proof, and verify the proof using drat-trim. 
Experiments were run on an Intel i7-3770 CPU machine running Ubuntu 16.04, with 32GB of RAM. 
The timeout for each instance is 129600 seconds (36 hours), and the result is shown in Table.~\ref{tab: RUC}

\begin{figure}
    \centering
    \begin{tabular}{ccc}
    \begin{minipage}{.33\linewidth}
    \begin{tabular}{||c |c | c  | c ||} 
 \hline
 S & SP & G & V \\  
 \hline\hline
 8.4 & 8.9 & 5.6 & 66.0 \\ 
 \hline
  2.6 & 2.5 & 2.9 & 20.4 \\
 \hline
  57.6 & 55.9 & 12.3 & 72.8 \\
 \hline
  1.7 & 1.6 & 2.5 & 13.8 \\
 \hline
  48.4 & 48.7 & 22.6 & 228.7 \\ 
 \hline
  1.15 & 1.20 & 2.22 & 4.83 \\
 \hline
  158.2 & 153.8 & 25.6 & 98.9 \\
 \hline
  7.6 & 7.8 & 4.20 & 49.7 \\
 \hline
  1.09 & 1.1 & 1.95 & 1.25 \\
 \hline
  0.20 & 0.23 & 1.0 & 0.52 \\
  \hline
  \multicolumn{4}{|c|}{$M=10$}\\
 \hline
\end{tabular}
    \end{minipage} &

    \begin{minipage}{.33\linewidth}
        \begin{tabular}{||c | c | c | c ||} 
 \hline
 S & SP & G & V \\  
 \hline\hline
119.69 & 121.2 & 105.3 & 14225.5 \\ 
 \hline
930.14 & 950.6 & 867.6 & 25944.4 \\
 \hline
8.46 & 8.7 & 47.6 & 349.6 \\
 \hline
2.86 & 2.9 & 58.6 & 1159.7 \\
 \hline
  1.88 & 2.0 & 45.9 & 457.5 \\ 
 \hline
  1.23 & 1.3 & 42.5 & 84.3 \\
 \hline
  36.1 & 36.0 & 61.7 & 989.8 \\
 \hline
  3.66 & 3.7 & 55.1 & 132.1 \\
 \hline
  0.37 & 0.38 & 33.7 & 106.8 \\
 \hline
  1.11 & 1.17 & 53.3 & 62.7 \\
   \hline
  \multicolumn{4}{|c|}{$M=20$}\\
 \hline
\end{tabular}
    \end{minipage} 
    \begin{minipage}{.33\linewidth}
        \begin{tabular}{||c | c | c | c ||} 
 \hline
 S & SP & G & V \\  
 \hline\hline
 1.9 & 2.0 & 351.8 & 2498.9 \\ 
 \hline
 8.16 & 8.2 & 339.8 & 767.0 \\
 \hline
  1141.2 & 1135.1 & 118757.9 & 580680\\
 \hline
  2.1 & 2.31 & 258.4 & 2711.6 \\
 \hline
  5.08 & 5.14 & 177.0 & 359.8 \\ 
 \hline
  0.68 & 0.73 & 240.3 & 837.4 \\
 \hline
  0.06 & 0.077 & 97.8 & 27.0 \\
 \hline
  0.23 & 0.29 & 94.7 & 64.0 \\
 \hline
  2.45 & 2.45 & 354.9 & 1729.7 \\
 \hline
   3.70 & 3.74 & 264.3 & 1394.1 \\
   \hline
   \multicolumn{4}{|c|}{$M=30$}\\
 \hline
\end{tabular}
    \end{minipage} 
\end{tabular}


    \caption{VLSI Routing Problem results. 
%
The three tables present the result of $M=10$, $M=20$, and $M=30$, respectively.
%
In each table, column $S$ records the MonoSAT solving time without proof, 
column $SP$ records MonoSAT solving time with proof, $G$ records the DRAT proof generation time, and $V$ records the DRAT proof verification time. 
%
All time are recorded in seconds.\lee{check why S<SP in M=30 table, row 3} }
    \label{tab:tab: RUC}
\end{figure}

The result indicates that our framework is capable of providing 
verifiable DRAT proofs for 29 of 30 UNSAT instances, and the online cost of MonoSAT to produce the casual proof certificate while solving is negligible (+/- 5\%). 
%
However, the scalability of our approach is challenged for DRAT proof generation and verification.
\lee{I'm confused why this is a criticism, if the verification uses drat-trim. I guess the point is the size of the proof-term?}
%
When $M \ge 20$, the cost of generating the full DRAT proof with the corresponding propositional definition for graph reachability is significant (100 times slower in the worst case) and increases with the size of the graph (i.e., $N$). 
%
This is due to the size of the monotone circuits for represent graph reachability. 
%
More specifically, the circuit size, in worst case, is roughly $M^2 * 4M^2$, which is $40000$ when $M=10$, $640000$ when $M=20$ and $3240000$ when $M=30$.
%
The grid-like shape makes the graph (and most of its subgraphs) cyclic and connective, making lemma-specific optimization (e.g., see remark~\ref{remark:reach} ) ineffective.  
%
The verification time of the full DRAT proof is comparable\lee{Be more precise?} with the proof generation time. 
%
The cost of verification depends on both the size of the input formula, which contains the propositional definition of reachability, and the size of the DRAT proof. 
%
As a result, verification is positively correlated with $M$ and the number of lemmas learned while solving, and is generally slower than the proof generation time. 
%
We observed the verification time is often 2 - 10 times slower than the proof generation time, and the ratio increases with $M$ as well. 
%
For graph reachability, the scalability issue is also caused by the size of monotone circuit. 
%
More specifically, given a monotone circuit of size $K$ for defining step-wise reachability definition, the number of unit propagation steps required to derive a theory lemma, in the worst case, is $O(K / 4)$, which is roughly $810000$ steps when $M=30$. 
. 
% However, we observed a few instances where the opposite holds.  
% The reasons are twofold: (1) the proof checker drat-trim is an optimized C program designed with performance in mind, while our proof generator is proof of concept written in python; (2) it might be sufficient to derive UNSAT with a small subset of reachability definition encoded by the proof generator. 

We observed that pruning irrelevant theory lemmas using \textsc{BackwardCheck} was effective in reducing the number of theory lemmas required for the DRAT proof. 
%
On average, 60\% of theory lemmas learned by MonoSAT were trimmed away. 

%For space reasons, the lemma specific status are not reported in Table.~\ref{tab:tab: RUC}, but they can be found in~\footnote{repoHolder}. 


==> workflow.tex <==
\section{Proof Support Workflow and Implementation}
\label{sec:workflow}
\sam{We will likely have to shrink or remove this section to make room for the Tiros results}
% In this section, we illustrate our framework for supporting DRAT proofs in MonoSAT. We first present the overall workflow for generating and verifying the DRAT-style UNSAT proof for MonoSAT, and then discuss the implementation details for the workflow.

  We instantiated our proof support framework for MonoSAT. 
%
The work flow is shown in Fig.~\ref{fig:workflow}. 
%
Given an input gnf instance (input formula for MonoSAT), we extended \textit{MonoSAT} to emit a DRAT-style proof certificate that contains theory lemmas (as explained in Sect.~\ref{sec:overview}). 
%
The proof certificate is then processed by \textit{drat-trim-theory}, a modified version of drat-trim running \textsc{BackwardCheck}, to extract the proof obligation. For every theory predicate whose predicate atom is in the proof obligation, the \textit{proof generator} encodes its propositional definition based on the predicate's monotone circuit (as shown in Sect.~\ref{sec:verifyTheory}). These definitions are used to expand the original theory predicates in the input formula to formulate an eq-satisfiable CNF formula. Finally, we use the unmodified drat-trim~\cite{DBLP:conf/sat/WetzlerHH14} to check the core lemmas (as a DRAT proof) on the CNF formula and return the verification result.
\pt{Did not introduce "gnf" before. It seems like an irrelevant detail that can be easily dropped without confusion.}

% The workflow for supporting the DRAT proof for MonoSAT is depicted in Fig.~\ref{fig:workflow}. Given an input gnf instance (input formula for MonoSAT), we extended \textit{MonoSAT} to emit a DRAT-style proof certificate that contains theory lemmas (as explained in Sect.~\ref{sec:overview}). The proof certificate is then processed by \textit{drat-trim-theory}, a modified version of drat-trim that runs Alg.~\ref{alg:check}, to extract the core lemmas, a subset of lemmas from the certificate which are sufficient as a DRAT proof if theory lemmas are assumed valid. For every theory predicate involved in the core lemmas, the \textit{proof generator} encode its propositional definition based on the predicate's monotone circuit (as shown in Sect.~\ref{sec:verifyTheory}). The propositional definitions for the predicates are then used to expand the original theory predicates in the gnf formula to formulate an eq-satisfiable CNF formula. Finally, we use the unmodified drat-trim~\cite{wetzler2014drat} to check the core lemmas (as a DRAT proof) on the CNF formula and return the result of the verification.

% The whole workflow can be broken down into three stages: (1) Solving with certificate (MonoSAT), (2) generating DRAT proofs (drat-trim-theory and proof generator), and (3) DRAT verification (drat-trim). We will evaluate their respective performance against the raw MonoSAT solving cost in Sect.~\ref{sec:evaluation}. 

\pt{I would rewrite the following paragraph dropping any reference to lines of code, which is a rather imprecise and uninformative measurement. It's more distracting than anything else.}
% To allow MonoSAT to emit proof certificate, we modified the solver with about 100 lines of C++ code. The solver supports emitting certificates in both plain text and binary mode. We implemented Alg.~\ref{alg:check} in drat-trim-theory by extending the drat-trim with less than 50 lines of C code. The proof generator was implemented with about 2000 lines of Python code that includes the monotone circuits for graph reachability and bit-vector comparison. 
%All tools are publicly available~\footnote{Place Holder}.


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{unsat_proof_wf.pdf}
    \caption{The workflow for generating and verifying DRAT proof for MonoSAT. Inputs to the workflow (instance gnf file and monotone circuits) are colored in blue. The new (proof generator) and modified components (MonoSAT and drat-trim-theory) are colored in yellow. The whole workflow can be broken down into three stages: (1) Solving with certificate (MonoSAT), (2) generating DRAT proofs (drat-trim-theory and proof generator) and (3) DRAT verification (drat-trim).}
    \label{fig:workflow}
\end{figure}

